RadArnomaly: Protecting Radar Systems from Data Manipulation Attacks

Radar systems are mainly used for tracking aircraft, missiles, satellites, and watercraft. In many cases, information regarding the objects detected by the radar system is sent to, and used by, a peripheral consuming system, such as a missile system or a graphical user interface used by an operator. Those systems process the data stream and make real-time, operational decisions based on the data received. Given this, the reliability and availability of information provided by radar systems has grown in importance. Although the field of cyber security has been continuously evolving, no prior research has focused on anomaly detection in radar systems. In this paper, we present a deep learning-based method for detecting anomalies in radar system data streams. We propose a novel technique which learns the correlation between numerical features and an embedding representation of categorical features in an unsupervised manner. The proposed technique, which allows the detection of malicious manipulation of critical fields in the data stream, is complemented by a timing-interval anomaly detection mechanism proposed for the detection of message dropping attempts. Real radar system data is used to evaluate the proposed method. Our experiments demonstrate the method's high detection accuracy on a variety of data stream manipulation attacks (average detection rate of 88% with 1.59% false alarms) and message dropping attacks (average detection rate of 92% with 2.2% false alarms).

==> sections/dataset.tex <==
\section{\label{sec:dataset}Dataset}

We rely on a dataset of benign radar behavior for the development of the anomaly detection mechanism. We use benign data collected from a real radar system deployed on different vessels to identify different objects. 
The data was collected from several different platforms at different times. 

The data contains in total 138,639 samples from 24 different recording sessions. 
The data was not uniformly distributed between the systems, and five recording sessions contains 76\% of the data (as can be seen in Figure~\ref{fig:RecordsDesc}).  
Therfore, for our evaluation we used these five recording sessions: R7, R19, R20, R29, R31.

\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{Fig/Records Description.png}
\caption{Records Description}
\label{fig:RecordsDesc}
\end{figure}

\subsection{\label{subsec:features description}Raw Features}
The data included 50 features. Table~\ref{tab:features} presents the features.
The features can be categorized as follows: 
\begin{enumerate}
\item constant (unchanged) features - eight of the features (such as srcid and msgid) were constant in the whole dataset. 
The reason is that in the collected dataset only one type of messages has been recorded, and all messages were from a single source (i.e., same radar entity used for each specific recording).
The recorded message type is the one used to inform the WCS about the objects that have been identified by the radar. This message type is considered the most important message type with regards to radar operation from a systems perspective. 
%please do not mention features that are not implemented
\item sequence-related - six features that should be evaluate while considering sequence of samples.
\item categorical - nine of the features were categorical, i.e., limited, fixed, number of possible values, with no mathematical metric. 
The following are examples for those categorical features: 
\begin{itemize}
    \item \textbf{trackCategory} - describes the object type, whether it airplane, cloud, etc.
    \item \textbf{hostility} - describes whether an object is an enemy or not. 
\end{itemize}
\item numerical - 18 of the features were numerical. The majority of these numerical features represent the correlation between the detected object's physical properties, i.e., the components of its location and speed vectors. 
\end{enumerate}

Note that the actual object location does not exist in our dataset due to information confidentiality.


\subsection{{\label{subsec:extracted}}Extracted Feature}

In addition to the raw (basic) features provided in the stream of events, we compute additional feature.  
We called this features $updatingPeriod$ and it's value is the UpdateTime difference between the current $Plot$ and the previous $Plot$ of the same $Track$ (e.g., $currentUpdateTime - prevUpdateTime$). 
For the first $Plot$ of the $Track$ the feature value is the same value as the second $Plot$ of the $Track$, since there is not $prevUpdateTime$. 
The main use of this feature is in tracking the time difference between $Plots$ so we can detect adding/drooping events.

The feature values vary and range from 100 to more then 1,000,000 time units. 
An histogram of this feature is presented in Figure~\ref{fig:updatingPeriod}.  

\begin{figure}[h]
\centering
\includegraphics[width=0.6\textwidth]{Fig/UpdatingPeriod histogram.png}
\caption{UpdatingPeriod histogram.}
\label{fig:updatingPeriod}
\end{figure}

\subsection{\label{subsec:plot tracks}Plots and Tracks}
Each sample in our dataset describes a $Plot$. 
A plot is a radar record that describes a detected object at a specific time. 
A plot record captures the object properties and radar-related metadata for the specific detection. 
Since the radar is continuously scanning the space, several plots may relate to the same object, describing properties of the same detected object at different times. 
A sequence of plots related to the same object is identified by the radar system as a $Track$.
Each track is indicated by a specific identification number (TrackID) in each plot record. 
In the datasets used, plots that appear within a specific recording session and have the same TrackID correspond to the same track. 
Figure~\ref{fig:plots_Tracks} present an illustration of plots (indicated by individual points) and a track (indicated by a sequence of connected points/plots).

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{Fig/Plots and Tracks.png}
\caption{Objects identified at a specific timestamp are represented by points. 
A sequence of points related to the same moving object are represented by a path of interconnected points (i.e., track).}
\label{fig:plots_Tracks}
\end{figure}

%Add a small example form the data


==> temp/backup-efrat.tex <==
\begin{comment}
We describe the complete detection procedure in Algorithm~\ref{alg:detection_process}.
The input to the detection procedure is a series of k+1 consecutive $Plot$ records that belong to the same $Track$ ($p_t$,$p_{t-1}$,...$p_{t-k}$) and three different thresholds ($th_1$, $th_2$, $th_3$). 

First, the $Plot$-level detection module is activated (lines 2-4) to compute the $p_t$ anomaly score (i.e., $pred_1$). 
If this score is higher than $th_1$, an alert is raised (lines 5-6). Then, the $Track$-level detection module is activated (line 7) to aggregate the $pred_1$ scores of $Plot$s that correspond to the same $Track$; this aggregation generates an anomaly score for the entire $Track$ (i.e., $pred_2$). 
If this score is higher than $th_2$, an alert is raised (lines 8-9). 

Finally, the $Sequence$-based detection module is activated (line 10) to compute an anomaly score for the $p_t$ arrival time (i.e., $pred_3$). If this score is higher than $th_3$, an alert is raised (lines 11-12). 

\begin{minipage}{.95\linewidth}
\begin{algorithm}[H]
\caption{Detection Procedure}\label{alg:detection_process}
%\small
\begin{algorithmic}[1]
\Function{Detect Anomalies}{$p_t$,$p_{t-1}$,...,$p_{t-k}$, $th_1$, $th_2$, $th_3$}
% \Statex\textit{Input:}
% \Statex $p$ - the current new $Plot$
% \Statex $p_6$ - six last $Plots$ corresponded to the same $Track$
% \Statex $t_1$, $t_2$, $t_3$ - three different thresholds
\State $categorical = ExctractCategoricalFeatures(p_t)$
\State $numerical = ExctractNumericalFeatures(p_t)$
%\State $embedding = Cat2Emb(categorical)$
\State $pred_1 = PlotLevelDetect(categorical, numerical)$
\If {$pred_1 > th_1$}
% \State \color{red}Rise Alert\color{black}
\State Raise Alert
\EndIf
%\State $PreprocessedData = DataPreprocess(p_t,p_{t-1},...,p_{t-k})$
\State $pred_2 = TrackLevelDetect(pred_1)$
\If {$pred_2 > th_2$}
% \State \color{red}{Rise Alert}\color{black}
\State Raise Alert
\EndIf
%\State $TracksScores = TrackAccumulate(pred_1)$
\State $pred_3 = SequenceBasedDetect(p_t,p_{t-1},...,p_{t-k})$
\If {$pred_3 > th_3$}
% \State \color{red}Rise Alert\color{black}
\State Raise Alert
\EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{comment}



%The following process was used to generate the test set: (1) given a benign dataset $B$, we first duplicate the benign dataset; (2) for each $Track$ $T$ in the duplicated benign dataset $B'$, we select a random location\footnote{\scriptsize The random location selected must be over a given threshold (e.g., five), since previous instances are needed in order to detect the attack. In addition, this number needs to be lower than $length(T) - 1$, since we need to keep the last $Plot$ at the end of $T$ for labeling.} in $T$; (3) from this random location, we count the number of packets there are until the last packet of the $Track$ and denote this number as $c$; (4) we drop a minimum number $minimum (c,10)$ of consecutive packets from the randomly selected location of $T$; (5) the event/$Plot$ that follows the dropped $Plot$ is labeled as an anomaly; and (6) we combine the test set $D_{test}$ and the duplicated, manipulated data into one test set.  
%We then drop the duplicates from the test set. This process generates a different number of benign and malicious events/$Plot$s; therefore the resulting test set is imbalanced.  



# system - the button --

\subsubsection{Plots and Tracks}
The radar system continuously communicates with the WCS and sends messages to it.
These messages include among other types, $Plot$ reports. 
$Plot$ describes the detected object properties at a specific time. 
Hence, it's considered to be the most important with regards to the radar operation from a systems perspective. 
Since the radar is continuously scanning the space, several $Plots$ may relate to the same object, describing properties of the same detected object at different times. 
A sequence of $Plots$ related to the same object is identified by the radar system as a $Track$.
Each $Track$ is indicated by a specific identification number (TrackID) in each $Plot$ record. 
%In the datasets used, plots that appear within a specific recording session and have the same TrackID correspond to the same track.
Figure~\ref{fig:plots_Tracks} present an illustration of plots (indicated by individual points) and a track (indicated by a sequence of connected points/plots).

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{Fig/Plots and Tracks.png}
\caption{Objects identified at a specific timestamp are represented by points. 
A sequence of points related to the same moving object are represented by a path of interconnected points (i.e., track).}
\label{fig:plots_Tracks}
\end{figure}

\subsubsection{Plot message fields}
Each $Plot$ update contains fields that describe (1) the message properties, (2) the identified object properties, and (3) sequence-related properties. 
The following is description of each one of them: 
\begin{itemize}
    \item message properties - message metadata, such as the source ID, message ID, message length, etc. 
    These fields are constant and do not change between $Plots$. 
    \item identified object properties - describe the object location, type, etc. 
    This properties could be divided into two group:  
    (1) categorical - limited, fixed, number of possible values, with no mathematical metric, such as, the object type which describes whether the identified object is an airplane, cloud, etc. 
    (2) numerical - unlimited numbers, with mathematical metric, these features mostly describe the object location and speed.
    \item sequence-related properties - have meaning only while considering a sequence of samples, such as updateTime, TrackID, etc.
\end{itemize}

A general radar system network can be connected to an organizational network, to a SCADA network that controls the utility services of the radar system (power, air condition, etc.), and in some scenarios to external entities over the Internet. 
Thus, this system is exposed either to internal or external threats.

In addition, for closed radar systems which are physically isolated and thus do not communicate with external entities, we consider the following threats as well: 
\begin{itemize}
    \item Possible insider threats - in many scenarios, the radar systems are integrated  
    
    \efrat{need to complete...}
    \item Supply-chain threats - if the attacker is a supplier of one of the radar system component, or even if he's a supplier of a system that is connected to the radar system, the radar system is in particular exposed to threats.
    \item Lack of security - due to the assumption that the radar system is a standalone system which is physically isolated from any external network, such a system tend not to include critical security countermeasures~\cite{c1}.
    \item Lack of software updates - from similar reasons mentioned above, software updates that contain vulnerability fixes are not installed. Those might be exploited by attackers.
    An example of the lack of software updates at the ECDIS (Electronic Chart Display and Information System) which often deployed on vessels and used to automatically navigate the ship could be shown in~\cite{c7}
    \item System complexity - in many scenarios, the radar systems are integrated into multi-system platforms hence many components are connected to the radar network.
    Thus, an attacker may take an advantage of this complexity and exploit many possibilities to connect his own device to the network in order to perform attacks. 
    \efrat{need to improve...}
\end{itemize}




In this section we provide with a brief description of the security aspects and threats as we presented in~\cite{cohen2019security}.

\textbf{Assets.} The assets of the radar systems that the attacker is interested in can be categorized as follows:
\begin{itemize}
    \item Physical assets: the physical components of the radar system (e.g. the antenna, the radar controller, etc.) 
    \item Computational units: the subsystems responsible for data analyzing; For example, the signal processor and the tracking algorithm. Both are part of the radar controller. Another example is the analyzing unit which is a part of the control system. 
    \item Data assets: the data present within the system (e.g. $Tracks$ or individual $Plots$).
    \item Connectivity assets: the physical components that are responsible for transferring data between physical components (e.g. the radar system network)
\end{itemize}

\textbf{Attacker Location.} The possible locations/positions of an attacker can be categorized as follows:
\begin{itemize}
    \item Physical access: the attacker has physical access to a physical asset of the radar system. In this case, the attacker can install malicious software or physically replace a legitimate device with a malicious device.
    \item Remote access: the attacker has access to the radar system via the Internet. In this case, the attacker can execute remote malicious commands on one or more of the radar system components.
    \item Close proximity: the attacker controls a device which is located near the antenna. The device has the ability to send signals at the radio domain.
    \item Supply chain: the attacker can execute a supply chain attack and compromise one or more of the components before the actual deployment.
\end{itemize}

\textbf{Threats.} The threats to radar systems are as follows:
\begin{itemize}
    \item Denial of service: harming the availability of a component of the radar system.
    \item Integrity violation: compromising the integrity of a component of the radar system and its data.
    \item Confidentiality violation: compromising the confidentiality of the data.
\end{itemize}


%%%%%%%%%%


\section{\label{sec:security}Radar Systems Security}

Very little research has been conducted on the security of radar systems. 
Although radar systems are vulnerable to a variety of threats~\cite{cohen2019security}, most of previous radar system related works focused on functionality aspects~\cite{barton2004radar,barton1988modern}.


The following are our assumption of the attacker possible locations/positions:  

\begin{itemize}
    \item Radar Controller (1) - the attacker has physical access to the radar controller. %during time periods in which the system is not in used (e.g., during maintenance). 
    Hence the attacker can install malicious software, replace one of the software components, or connect his/her malicious device. 
    
    \item Radar system network (2) - the attacker has physical access to the radar system network, hence the attacker can replace the network switch, and/or connect his/her malicious device. %A possible attack from this position, for example, can be in the form of radar spoofing, i.e., with a malicious device pretending to be the legitimate radar, transmitting messages to the WCS instead of or alongside the authentic radar entity.
    
    \item External network (3) - the attacker has physical access to the external network of the radar. 
    Hence the attacker can exploit vulnerabilities in one of the radar components in order 
\end{itemize}  

The effects of such tampering activity are expected to be covert; and, specifically, to be "under the radar" for the radar operators (i.e., radar operators should not be able to identify the tampering).

Based on the above, we place our anomaly detector between the radar system network to the CS. 




%%%%%%%%%%
Our proposed method consists of the following three stages:

(1) Data modeling - we utilize state of the art machine learning methods to model the data in order to be able to identify anomalies that potentially provide indications for a cyber attack. 
(2) Anomalies creation - we analyze how the possible attack scenarios can be reflected in the data, and create a set of anomalous data accordingly. 
(3) Model evaluation - we evaluate the model ability to distinguish between the created anomalous data and the benign data. 


%%%%%%%%%%
\subsection{{\label{subsec:extracted}}Extracted Feature}

In addition to the raw (basic) features provided in the stream of events, we compute additional feature.  
We called this features $updatingPeriod$ and its value is computed using the feature $UpdateTime$. 
This feature indicate of the $UpdateTime$ difference between the current $Plot$ and the previous $Plot$ of the same $Track$ (e.g., $currentUpdateTime - prevUpdateTime$). 
For the first $Plot$ of the $Track$ we set the feature value to be the same value as the second $Plot$ of the $Track$, since for the first $Plot$ in the $Track$ there is no $prevUpdateTime$. 
The main use of this feature is in tracking the time difference between $Plots$ so we can detect drooping events.

The feature values vary and range from 100 to more than 1,000,000 time units, this indicates that just setting a threshold on this feature could not be a good strategy for detecting a drooping events. 
An histogram of this feature is presented in Figure~\ref{fig:updatingPeriod}.  

\begin{figure}[h]
\centering
\includegraphics[width=0.6\textwidth]{Fig/UpdatingPeriod histogram.png}
\caption{UpdatingPeriod histogram.}
\label{fig:updatingPeriod}
\end{figure}


\subsection{\label{subsec:model}Data Modeling}

\subsubsection{Model high level architecture}

The proposed model consist of the following two main phases, (presented in Figure~\ref{fig:HLA}): (1) Modeling of the $Plot$ structure. (2) Modeling of a sequence time intervals. 
Following is a detailed description of the two phases.


\subsubsection{Modeling of the $Plot$ structure.}
The main goal of this phase is to examine whether the relation between the different features of the $Plot$ is similar to the relation that has been learned from benign $Plots$. 
This phase is consist of the following three stages. (1) Categorical to numerical embedding, (2) plot-level point anomaly detector, and, (3) track-level anomaly detector. 
In the next subsections we will describe each one of them. 

\subsubsection{Categorical to numerical embedding}
%One of the most famous ways to deal with categorical data is by using a one-hot-encoding representation.  
%According to this representation, each categorical feature is converted to a vector that is as long as the number of possible values of this feature. 
%This vector has a value of one in one place, corresponding to the actual feature value, and zeroes in the rest, so each unique value has a unique vector representation.
%This method suffers from two main drawbacks: (1) This representation do not capture the relation between categorical variables. (2) The created representation could suffer from curse of dimensionality. 

AutoEncoder embedding representation is commonly used to create a short representation for categorical features~\cite{hancock2020survey}. 
\shai{TODO: maybe need to explain about AutoEncoder}
Using this method an AutoEncoder is trained and the Encoder output is used as a representation of the input data. 

One of the most famous example is Word2Vec technique which used in the natural language processing domain~\cite{c4}. (\shai{TODO: shai - maybe we need to drop this sentence.})

%Using the Word2Vec technique each word (or token) is represented using a numerical vector that preserves the semantic relations between words.
%For example, in the natural language processing (NLP) domain an Word2Vec model will learn that the distance between the vectors representing \textbf{king} and \textbf{man} is similar to the distance between the vectors representing \textbf{queen} and \textbf{women}. 
%This means that the algorithm gives the same relation between words analogically are similar. 
%In many scenarios (such as Word2Vec) the categorical features represent the same entity (e.g., the word in different locations in the sentence), but in many others, it describes different entities (e.g., our case) so the relation between them is unknown. 
In our anomaly detection model, we utilize a similar method called Cat2Emb.
The categorical features in our data are multi-field features. which means that the relation between them is unknown.
Therefore, our designed Cat2Emb model was inspired by the models presented in~\cite{c5}~\cite{c6}. 

The architecture of the Cat2Emb model, (presented in Figure~\ref{fig:cat2emb}), includes three parts:

\begin{enumerate}
    \item In the first part, there is a separate embedding layer for each of the categorical features. 
    This embedding layer gets one integer as input and output one number. 
    The number of possible values for the inputted integer is the number of possible values of the corresponding categorical feature \footnote{In some of the categorical features we shift the values before inputting them to the model, so the minimum values will be zero}.
    
    The embedded layer works in the following way: 
    A one-hot-encoding representation/vector is created for the inputted value,
    This representation/vector is multiplied with a corresponded weights vector (W) and returned the single output value.
    \item In the second part, the nine outputs from the nine separate embedding layers are concatenated, creating a vector with a length of nine. 
    \item In the third part, the concatenated vector is fully connected to nine separate vectors. 
    Each of these nine vectors corresponds to a different feature. 
    For this reason, the size of each of these nine vectors is equal to the number of possible values of the corresponded categorical feature.
    The activation function used in this layer is Sigmoid. 
\end{enumerate}    
    
%As an example, TrackGrade has 4 possible values, then the corresponding embedding layer will have 4 possible inputs. 
%The output dimension is 1 in all of the embedding layers.  
%This layer is acting as a lookup table so for every possible value it matches its corresponding value in the table. 

As the input for the Cat2Emb network is a vector in a length of nine, the network goal is to reconstruct the values of the input vector such that there will be "1" in a single place in each of the 9 output vectors and "0" in all the other places.
In each output vector the "1" location is related to the input value in the correspond input.
To do so, we trained the network to minimize the SparseCategoricalCrossEntropy measure using Adam optimizer~\cite{c2}. 
The global network loss is a sum of the loss of all of the nine final vectors.

In the resulting network, the concatenated vector is used as the embedding space (numerical) representation for the categorical features.
In this vector, each categorical feature is contribute to more then one element. 
The intuition for this is as follows:
Each of the embedding layers represents several one-hot-encoding vectors by using only one number, then using these numbers the network tries to reproduce each of the inputs and present it using one-hot-encoding representation.
The network could not use only the one number created by a one embedding layer to reproduce its one-hot-encoding representation since the transformation from one number to several orthogonal vectors is not linear. 
Therefore, to reproduce each of the one-hot-encoding vectors the network use more than one number. 

%To do so, the network tried to find relations between appeared set of values, so maybe several sets are similar to each other and this create a vector with a mathematical relations. 

\begin{figure*}[h]
\centering
\includegraphics[width=1.1\textwidth]{Fig/Embedding Representation.png}
\caption{Cat2Emb}
\label{fig:cat2emb}
\end{figure*}

\subsubsection{Plot-level anomaly detector}
By using the embedding representation for the categorical features created by the Cat2Emb model together with the numerical features, we use a stack autoencoder (AE) model for detecting anomalous plots. 
The architecture of the this AE is presented in Figure~\ref{fig:fullModel}.

As can be seen, first, the embedding representation of categorical features (computed by the Cat2Emb model) is concatenated with the numerical features, resulting in a vector of size 27.
Then, a min-max scaler is applied to this vector to normalize all features.
Then, the normalized vector is fed into the stacked AE consisting of seven layers with 27, 20, 15, 10, 15, 20, 27 neurons respectively.
In all neurons the activation function used is Sigmoid.

The AE is trained using the training set to minimized  the mean square error measure (MSE) using Adam optimizer.

%Once the model is trained, it is applied on a validation set in order to determine the detection threshold.
%One common approach for determining the detection threshold is using the max MSE value observed by applying the model on the samples of the validation set.
%Then, an alert will be raised for samples in the test set for which the MSE value exceeds the selected anomaly detection threshold.

\begin{figure}[h]
\centering
\includegraphics[width=0.9\textwidth]{Fig/Full Model.png}
\caption{Full Model}
\label{fig:fullModel}
\end{figure}

\subsubsection{Tracks anomaly detector.} 
In most scenarios, the attacker gets a much greater benefit if he/she changes a feature of $Plots$ for the entire $Track$.
For example, an attacker who wants to change the type of the object identified by the radar (e.g., TrackCategory) so it will not be classified as an aircraft would prefer to do so for the entire $Track$.
The reason is that changing the object type for only several $Plot$ of the $Track$ has less influence in deciding which action should be taken, at the same time, the change of this feature during the $Track$ is not supposed to happen, and is very suspicious. 
%TODO: shai - explain it better.
For this reason it is more accurate and will cause less false positives if the threshold will be decided by the mean loss of the $Track$, hence in this stage we calculate the mean loss to decide whether a feature is changed in a $Track$.
\shai{TODO: shai - maybe declare that this is another detection method.}

\subsubsection{Modeling of a sequence time intervals}
A $Plot$ that has been tested so none of its features have been changed is forward to the model second phase.
In this phase, we model the time between packets and try to understand whether the arrival time of the packet is legitimate. 
This is done using the following two stages. (1) Data processing. and, (2) Sequence anomaly detector. 
In the next subsections we will describe each one of them. 

\subsubsection{Data processing}
At this stage, we concatenate the previous six $Plots$ of the same $Track$ as the current $Plot$ along with the current $Plot$, hence creating a sequence of a length of 7. 
In this sequence we use five features, TargetRT, trackGrade, quality, trackCategory, and updateTime and process the data in the following way: 
(1) Encode the categorical features (i.e., trackGrade, quality, trackCategory) using one-hot-encoding. 
(2) Extract UpdatingPeriod using updateTime. 
(3) Drop the first element of the sequence ending up with sequence in a length of 6. 
(4) Apply min max scaler on the data for feature scaling. 
(5) take the 5 first element of the sequence to be the input for the model and the value of $updating period$ feature of the sixth element to be the expected/predicted value. 

\subsubsection{Time interval anomaly detector}
Long Short Term Memory (LSTM) networks are well-known deep learning networks that are very suited for sequential data. 
In this type of network instead of processing the whole sequence together, the network process each object of the sequence separately in chronological order. 
So in each step, the network inputs are: (1) the current object in the sequence, together with the (2) output of the network from the previous step. 

By using an LSTM component we design a simple LSTM based regressor.
This LSTM regressor gets as an input the processed sequential data created in the previous stage and predict the $updating period$ (e.g., time interval) value of the next $Plot$ of the sequence. 

The architecture of this regressor is presented in Figure~\ref{fig:lstm}. 
As can be seen, the 5 length sequence is inputted into an LSTM network with 5 hidden units. 
The output of the LSTM component at the final step is fully connected to one neuron. 
At the end, a Sigmoid activation function is applied on this neuron. 
The network is trained using the training set to minimized the mean square error measure (MSE) using Adam optimizer.

\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{Fig/LSTM network.png}
\caption{LSTM based regressor}
\label{fig:lstm}
\end{figure}

\shai{TODO: shai - add a section to explain how we give score to samples.}

%For the evaluation, we used the five recording sessions that contain the most data (presented in ~\ref{fig:RecordsDesc}).
We conducted the following three types of evaluations:
\begin{itemize}
    \item \textbf{Cross-session setup:} in this case, each time we used four recording sessions for training and the fifth remaining session was used for testing the model.
    
    \item \textbf{Chronological setup:} in this case, for each recording session we train the model on the first 90\% instances (by chronological order) and test it on the remaining 10\% instances.
    
    \item \textbf{Transfer learning setup:} this case is a combination of the previous two setups in which we used four recording sessions as well as the first 10\% of the instances of the fifth session for training the model, and the remaining 90\% instances of the fifth session were used for testing the model. 
\end{itemize}

In all of these cases we repeated the experiments five time (each time a different recording session was selected for testing).
For example, in a scenario in which the examine session is R5, the following are the train and test data in each evaluation setup: 
\begin{itemize}
    \item \textbf{Cross-session setup:} train -  R1, R2, R3 and R4 ; test - R5. 
    \item \textbf{Chronological setup:} train - 90\% of first instances in R5 ; test - remaining 10\% instances of R5. 
    \item \textbf{Transfer setup:} train -  R1, R2, R3, R4 and first 10\% instances of R5 ; test - remaining 90\% instances of R5.
\end{itemize}

\shai{TODO: combine the above two items}

















%%%%%%%%%%%%%%%%%%




\section{\label{sec:evaluation}Evaluation}
In order to evaluate the models, we implemented four attack scenarios and conducted 15 different experiments for each attack.  

\subsection{\label{subsec:dataset}Benign Dataset for Training}

For the evaluation we use benign data collected from five real radar systems which are deployed on different operational setups and used for identifying objects. 
We refer to each dataset as a \emph{recording session}.
The number of messages in each recording session is as follows: R1 -- 45,720 (43\%), R2 -- 23,017 (21.7\%), R3 -- 15,992 (15.1\%), R4 -- 11,955 (11.2\%), and R5 -- 9,551 (9\%). %presented in Table~\ref{tab:dataset}.
In total, there are 106,235 messages.

\begin{comment}
\begin{table}[h!]
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Recording session} & \textbf{Number of messages} & \textbf{Percentage} \\ 
\hline
R1 & 45,720   & 43\% \\ \hline
R2 & 23,017    & 21.7\% \\ \hline
R3 & 15,992    & 15.1\% \\ \hline
R4 & 11,955    & 11.2\% \\ \hline
R5 & 9,551    & 9\% \\ \hline
\end{tabular}
\caption{Dataset description.}\label{tab:dataset}
\end{table}
\end{comment}

\subsection{\label{subsec:attacks} Attack Scenarios Implemented}
A labeled testset which includes both benign and malicious samples is needed to evaluate the proposed model.
Since our dataset does not include any attacks, we had to simulated the attacks and inject them into our dataset.
In the evaluation we focused on two classes of attacks that an attacker could benefit from.

\subsubsection{Categorical feature manipulation.} 
This is an integrity attack in which the attacker changes one categorical feature. 
% We implemented this attack on the features (1) trackCategory, (2) hostility, and (3) threatAlert, 
% We chose these features since manipulation of these features can help an attacker avoid detection from the radar system/system operators which is one of the most significant goals an attacker may want to achieve.
Changes in the following features may cause the consuming system to characterize and handle the detected object incorrectly.
\begin{itemize}
    \item trackCategory - in this scenario, the attacker changes the category of the object, such that air objects will be seen as ground objects and vice versa. 
    This may change the way the radar operator is reacting to the different objects and may help an attacker be left untreated by the radar operator.
    \item threatAlert - in this scenario, the attacker change the hostility level identified by the radar, such that friend object will be seen as foe objects, etc. 
    This attack may case the radar operators to fire on friend objects or ignore enemy objects.
    \item hostility - in this scenario, the attacker change the alert that will be raised as a result of object identification, such that alert will not raised when needed and vice versa, 
    This attack may create many false alarms and may also cause the radar operator to ignore foe objects.
\end{itemize}

%Manipulating features such as trackGrade, trackRCSectimation, burnTrough, multipath, quality, and plotRangeRateValidity will result in reducing the confidence of the system in the interpretation of the detected object.

Changing features for an entire $Track$ or a $Track$ segment will be much more beneficial to the attacker than changing features for random $Plots$. 
This is because changes in the features of random $Plots$ may be ignored by the radar operator and are not likely to influence the action taken by an operator. 
Therefore, in this attack scenario, we evaluate our model against changes in the entire $Track$. 

The following process was used to generate the attack: (1) given a test set $D_{test}$, we first duplicate the test set; (2) in the duplicated test set, for an examined (manipulated) feature $f$ for each track $t$, we change the value of $f$ \shai{to a possible value occurred least in the $t$}, for the whole track; (3) we label the manipulated events/plots as anomalies; and (4) we combine the test set $D_{test}$ and the duplicated, manipulated data into one test set.  
This process generates a similar number of benign and malicious events/plots; therefore, the resulting test set is balanced. 

\subsubsection{Drop plots.} Dropping of one/several plots from a track, so that the consuming system will be less confident in the track/object that has been detected. 

The process for creating this attack is as follows: 
(1) given a test set $D_{test}$, we first duplicate the test set; (2) for each track $t$ in the duplicated test set, we select a random location\footnote{The random location selected must be over a given threshold (e.g., five), since previous instances are needed in order to detect the attack. In addition, this number needs to be lower than $length(t) - 2$, since we need to keep the last plot at the end of $t$ for labeling.} in $t$; (3) from this random location, we count the number of packets that there are until the last packet of the Track and denote this number as $c$; (4) we drop a number of $minimum(c,10)$ consecutive packets from the randomly selected location of $t$; (5) the event/plot that follows the dropped plots is labeled as an anomaly; and (6) we combine the test set $D_{test}$ and the duplicated, manipulated data into one test set.  
From this test set, we drop duplicates. 
This process generates a different number of benign and malicious events/plots; therefore the resulting test set is imbalanced.  


\subsection{\label{subsec:evalsetup}Evaluation Method}

We conducted three types of evaluations; in each case, we repeated the experiments five times (each time a different recording session was selected for testing).
A description of the types of evaluations performed is provided below, along with an example of the training/testing data in a scenario in which the R5 session is examined: 
\begin{itemize}
    \item \textbf{Cross-session setup:} in this case, each time we used four recording sessions for training, and the fifth session was used to test the model. 
    Example for the R5 session: training -  R1, R2, R3, and R4; testing - R5. 
    \item \textbf{Chronological setup:} in this case, for each recording session, we trained the model on the first 90\% of the instances (in chronological order) and tested it on the remaining 10\% of the instances.
    Example for the R5 session: training - 90\% of the instances of R5; testing - remaining 10\% of the instances of R5.
    \item \textbf{Transfer learning setup:} this case is a combination of the previous two setups, in which we used four recording sessions, as well as the first 10\% of the instances of the fifth session to train the model, and the remaining 90\% of the instances of the fifth session were used to test the model. 
    Example for the R5 session: training -  R1, R2, R3, R4, and the first 10\% of the instances of R5; testing - the remaining 90\% of the instances of R5.
\end{itemize}
\shai{It should be noted that the cross-session evaluation setup has two significant advantages over the other two: (1) in practice, it is easier for radar engineers to deploy a model that has already been trained rather than training a model using the new system data, and (2) training the model on the new system data can expose the model to cyber risk (e.g., adversarial poisoning ~\cite{vorobeychik2018adversarial}).}

\subsection{\label{subsec:evalmetric}Evaluation Metrics}

The task of identifying anomalies in the radar data stream is a classification task, where benign samples are labeled as zero (negative), and malicious data is labeled as one (positive).
We used the following common metrics for the evaluation: True Positive Rate (TPR)/Recall, False Positive Rate (FPR), Receiver Operating Characteristic (ROC) Curve, Area Under the ROC Curve (AUC), Precision, Precision-Recall Curve, and average precision (AP).

\begin{comment}
\begin{itemize}
    \item \textbf{True Positive Rate (TPR)/Recall} - the ratio of the number of malicious samples identified by the model that are actually positive (TP) to the total number of malicious samples in the test data (P).   
    \item \textbf{False Positive Rate (FPR)} - the ratio of the number of benign samples that were misclassified by the model (FP) as malicious to the total number of benign samples in the test data (N). 
    \item \textbf{ROC (Receiver Operating Characteristic) Curve} - since the model returns the probability for a sample to be malicious, the number of benign/malicious samples predicted by the model is dependent on the probability threshold. 
    When this threshold increases, the TPR increases and the FPR decreases, and vice versa.
    The ROC curve represents the relation between the TPR to the FPR for different thresholds.  
    \item \textbf{AUC (Area Under Curve)} - the area under the ROC curve; a number ranging from zero to one that represents the model quality. 
    \item \textbf{Precision} -  the ratio of the number of malicious samples identified by the model that are actually positive (TP) to the total number of samples that were predicted by the model to be positive (TP + FP). 
    \item \textbf{PRC (Precision Recall Curve)} - represents the relation between the $Precision$ to the $Recall$ for different thresholds.  
    \item \textbf{AP (Average Precision)} - weighted mean of the $Precision$ for each threshold, i.e., $\sum_n(R_n - R_{n-1})*P_n$; a number ranging from zero to one that represents the model quality. 
\end{itemize}
\end{comment}

\subsection{\label{subsec:results}Results}
The following are the results for each attack scenario: 

\textbf{Categorical feature manipulation attack results.}
We evaluate the purposed model ability to detect manipulation attacks on the features (1) trackCategory, (2) hostility, and (3) threatAlert, 
We chose these features since manipulation of these features can help an attacker avoid detection from the radar system/system operators which is one of the most significant goals an attacker may want to achieve.
In these scenarios, the test set is balanced (i.e., contains similar number of malicious and benign samples/$Tracks$).


\textbf{Manipulating of trackCategory.}
Figure~\ref{fig:trackCategory} present the detection results of the track-level detection module on this attack. 

%As could be noticed, in most scenarios the model achieved significant results. 
%The only scenario in which the model performance was less good is the Chronological test by using R3 as the recording session.

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Fig/Evaluation Results - Change Feature - trackCategory.png}
\caption{The ROC and PRC curves for the trackCategory change feature attack for each session examined.}
\label{fig:trackCategory}
\end{figure}

\textbf{Manipulating of hostility.}
Figure~\ref{fig:hostility} present the detection results of the track-level detection module. 

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Fig/Evaluation Results - Change Feature - hostility.png}
\caption{The ROC and PRC curves for the hostility change feature attack for each session examined.}
\label{fig:hostility}
\end{figure}

\textbf{Manipulating of threatAlert.}

Figure~\ref{fig:threatAlert} present the detection results of the track-level detection module. 

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Fig/Evaluation Results - Change Feature - threatAlert.png}
\caption{The ROC and PRC curves for the threatAlert change feature attack for each session examined.}
\label{fig:threatAlert}
\end{figure}

%\subsubsection{Inject plots attack results}

\textbf{Drop packets attack results.}
Table~\ref{tab:drop_packet} present the distribution of the benign/malicious samples in the drop packet attack. 
It's could be noticed that the data is imbalanced, since for each $Track$ we execute the attack only once. 
The performance of the Time interval detection module on the generated dataset is presented in Figure~\ref{fig:drop_packet}
As could be noticed, in all scenarios the model achieved significant results. 

\begin{table}[h]
\centering
\small
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{}             & \multicolumn{10}{c|}{\textbf{Session Examined}}                                                                      \\ \cline{2-11} 
                              & \multicolumn{2}{c|}{\textbf{R1}}     & \multicolumn{2}{c|}{\textbf{R2}}     & \multicolumn{2}{c|}{\textbf{R3}}
                              & \multicolumn{2}{c|}{\textbf{R4}}
                              & \multicolumn{2}{c|}{\textbf{R5}}\\ \hline
                              & \textbf{b} & \textbf{m} & \textbf{b} & \textbf{m} & \textbf{b} & \textbf{m} &
                         \textbf{b} & \textbf{m} & \textbf{b} & \textbf{m}\\ \hline
Cross Directories    & 46,600          & 213                  & 23,068               & 177                  & 16,237               & 122  & 12,139 & 97 & 9,484 & 119             \\ \hline
Chronological (10\%) & 4,606               & 60                  & 2,323               & 34                  & 1,609               & 24 & 1,206 & 15 & 842 & 31               \\ \hline
Transfer (90\%)      & 42,709 & 195  & 21,126     & 170                  & 14,660               & 105 & 10,808 & 86 & 8,451 & 110                 \\ \hline

\end{tabular}
\caption{Drop packet benign (b) and malicious (m) number of samples.}
\label{tab:drop_packet}
\end{table}

% \begin{comment}
% \begin{table}[]
% \centering
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% \multirow{2}{*}{}             & \multicolumn{4}{c|}{\textbf{Session Examined}}                               \\ \cline{2-5} 
%                               & \multicolumn{2}{c|}{\textbf{R4}}     & \multicolumn{2}{c|}{\textbf{R5}}     \\ \hline
%                               & \textbf{benign} & \textbf{malicious} & \textbf{benign} & \textbf{malicious} \\ \hline
% Cross Directories    & 12,139          & 97                  & 9,484               & 119                  \\ \hline
% Chronological (10\%) & 1,206               & 15                  & 842               & 31                  \\ \hline
% Transfer (90\%)      & 10,808               & 86                  & 8,451               & 110                  \\ \hline
% \end{tabular}
% \caption{Drop packet benign/malicious number of samples.}\label{tab:drop_packet}
% \end{table}


% \begin{table}[]
% \centering
% \scriptsize
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{}             & \multicolumn{6}{c|}{\textbf{Session Examined}}                                                                      \\ \cline{2-7} 
%                               & \multicolumn{2}{c|}{\textbf{R1}}     & \multicolumn{2}{c|}{\textbf{R2}}     & \multicolumn{2}{c|}{\textbf{R3}}     \\ \hline
%                               & \textbf{benign} & \textbf{malicious} & \textbf{benign} & \textbf{malicious} & \textbf{benign} & \textbf{malicious} \\ \hline
% Cross Directories    & 46,600          & 213                  & 23,068               & 177                  & 16,237               & 122                \\ \hline
% Chronological (10\%) & 4,606               & 60                  & 2,323               & 34                  & 1,609               & 24                  \\ \hline
% Transfer (90\%)      & 42,709               & 195                  & 21,126               & 170                  & 14,660               & 105                  \\ \hline
% \end{tabular}
% \end{table}


% \begin{table}[]
% \centering
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% \multirow{2}{*}{}             & \multicolumn{4}{c|}{\textbf{Session Examined}}                               \\ \cline{2-5} 
%                               & \multicolumn{2}{c|}{\textbf{R4}}     & \multicolumn{2}{c|}{\textbf{R5}}     \\ \hline
%                               & \textbf{benign} & \textbf{malicious} & \textbf{benign} & \textbf{malicious} \\ \hline
% Cross Directories    & 12,139          & 97                  & 9,484               & 119                  \\ \hline
% Chronological (10\%) & 1,206               & 15                  & 842               & 31                  \\ \hline
% Transfer (90\%)      & 10,808               & 86                  & 8,451               & 110                  \\ \hline
% \end{tabular}
% \caption{Drop packet benign/malicious number of samples.}\label{tab:drop_packet}
% \end{table}
% \end{comment}


% \begin{table}[h!]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{}    & \multicolumn{5}{c|}{\textbf{Examine session}}                       \\ \cline{2-6} 
%                      & \multicolumn{1}{c|}{\textbf{R1}} & \multicolumn{1}{c|}{\textbf{R2}} & \multicolumn{1}{c|}{\textbf{R3}} & \multicolumn{1}{c|}{\textbf{R4}} & \multicolumn{1}{c|}{\textbf{R5}} \\ \hline
% Cross Directories    & 46,600/213 & 23,068/177 & 16,237/122 & 12,139/97 & 9,484/119\\ \hline
% Chronological (10\%) & 4,606/60 & 2,323/34 & 1,609/24 & 1,206/15 & 842/31\\ \hline
% Transfer (90\%)      & 42,709/195         & 21,126/170         & 14,660/105         & 10,808/86         & 8,451/110\\ \hline
% \end{tabular}
% \caption{Drop packet benign/malicious number of samples.}\label{tab:drop_packet}
% \end{table}


%In this scenario, we apply the drop packets attack to the data, then we evaluate the model's ability to detect the samples that have been labeled as anomalies (i.e., a one-sample in the $Track$ that appears after the sequence of the drooped packets).
%To do so, after applying the attack we calculate the feature $updatingPeriod$, this feature 

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Fig/Evaluation Results - Drop Packet.png}
\caption{The ROC and PRC curves for the drop packet attack for each session examined.}
\label{fig:drop_packet}
\end{figure} 

\textbf{Setting threshold.}
\shai{We set two thresholds that achieved FPR of 0.01 and 0.05, then for each attack scenario, we averaged the TPR on the five experiments.
The results are presented in Table~\ref{tab:results_summary}.}

\shai{It's could be noticed that the model successfully classify almost all of the drop packets attack even when allowing a FPR of 0.01 and most of the change feature attacks when allowing FPR of 0.05.}

\shai{In the drop packets attack, there is no much difference between the different evaluation setups.
In the change feature attack when allowing FPR of 0.01, the models that trained in the cross directories setup, achieved competitive results compared to the two other setups.
And when allowing an FPR of 0.05, these models achieved even better results compared to the two other setups.
This may indicate that (1) the data created for the different sessions has a very similar distribution.
(2) Some of the samples in the new tested session are from a distribution that is different from the other sessions, hence they are more likely to be labeled as malicious by the model that is trained in the cross sessions setup.
In conclusion, based on our results, we suggested to train the model on the different systems and to not retrain it on the new system.}

\begin{table}[h]
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\small
\textbf{Attack scenario} & \textbf{Test type}   & \textbf{\begin{tabular}[c]{@{}l@{}}Average TPR \\ (FPR=0.01)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Average TRP \\ (FPR=0.05)\end{tabular}} \\ \hline
Change feature - trackCategory & Cross directories    & 0.38                                                                       & 0.75                                                                        \\ \hline
Change feature - trackCategory & Chronological (10\%) & 0.25                                                                       & 0.48                                                                        \\ \hline
Change feature - trackCategory & Transfer (90\%)      & 0.25                                                                       & 0.56                                                                        \\ \hline
Change feature - hostility     & Cross directories    & 0.15                                                                       & 0.48                                                                        \\ \hline
Change feature - hostility     & Chronological (10\%) & 0.3                                                                        & 0.63                                                                        \\ \hline
Change feature - hostility     & Transfer (90\%)      & 0.22                                                                       & 0.52                                                                        \\ \hline
Change feature - threatAlert   & Cross directories    & 0.34                                                                       & 0.81                                                                        \\ \hline
Change feature - threatAlert   & Chronological (10\%) & 0.52                                                                       & 0.65                                                                        \\ \hline
Change feature - threatAlert   & Transfer (90\%)      & 0.61                                                                       & 0.61                                                                        \\ \hline
Drop packets                   & Cross directories    & 0.88                                                                       & 0.97                                                                        \\ \hline
Drop packets                   & Chronological (10\%) & 0.92                                                                       & 0.99                                                                        \\ \hline
Drop packets                   & Transfer (90\%)      & 0.89                                                                       & 0.95                                                                        \\ \hline
\end{tabular}
\caption{\shai{The average TPR for each attack scenario when setting a threshold such that it achieved FPR is 0.01 and 0.05.}}\label{tab:results_summary}
\end{table}
